Image Inpainting for High-Resolution Textures using CNN Texture Synthesis

Deep neural networks have been successfully applied to problems such as image segmentation, image super-resolution, coloration and image inpainting. In this work we propose the use of convolutional neural networks (CNN) for image inpainting of large regions in high-resolution textures. Due to limited computational resources processing high-resolution images with neural networks is still an open problem. Existing methods separate inpainting of global structure and the transfer of details, which leads to blurry results and loss of global coherence in the detail transfer step. Based on advances in texture synthesis using CNNs we propose patch-based image inpainting by a CNN that is able to optimize for global as well as detail texture statistics. Our method is capable of filling large inpainting regions, oftentimes exceeding the quality of comparable methods for high-resolution images. For reference patch look-up we propose to use the same summary statistics that are used in the inpainting process.

==> discussion.tex <==
\section{Discussion} \label{sec:disc}
As presented in Sec. \ref{sec:results} our method is able to inpaint high-resolution texture satisfying global structure as well as details.
While surpassing other methods in terms of maintaining texture statistics results may contain color deviations in-between inpainted patches depending strongly on reference patch selection.
This especially is the case when the source region $\Phi$ has a very diverse color palette like the example in Fig. \ref{fig:bricks}.
Using the difference of masked Gramians as a metric for patch distance has major benefits for our inpainting approach over using simple MSE.
Since we are not dependent on reference textures $\x_d$ or $\x_g$ exactly matching $\Psi$ inside $\hat{\x}_d$ or $\hat{\x}_g$ in terms of MSE, we can reduce the number of samples taken from $\Phi$ in reference patch look-up.
MSE is not well suited as a measure of texture similarity as can be seen from the result of EBI for inpainting the \textit{Bricks} example texture.
While achieving the lowest value for MSE, the approach fails when examined visually.
Due to the averaging of feature information inside Gramians, global spacial information is lost.
This enables the Gramian to represent texture invariant to rotation and translation to some degree (see Fig. \ref{fig:references}).
Because our loss term $\Lb$ is based on the difference of Gramians this further ensures that $\Psi$ inside $\hat{\x}$ already satisfies target statistics to some extent.
\begin{figure}[htb!]
\centering
\subfloat[]{
		\includegraphics[width=0.15\textwidth]{images/inp_reg.jpg}
\label{fig:polka7}
}
\subfloat[]{
		\includegraphics[width=0.15\textwidth]{images/inp_ref.jpg}
\label{fig:polka8}
}
\subfloat[]{
		\includegraphics[width=0.15\textwidth]{images/inp_res.jpg}
\label{fig:polka9}
}
\caption{\protect\subref{fig:polka7} Inpainting patch $\hat{\x}_d$. \protect\subref{fig:polka8} Closest reference patch from $\Phi$. \protect\subref{fig:polka9} Inpainting result.}
\label{fig:references}
\end{figure}

Major strength of our method is the correct inpainting of global structure while also maintaining details.
When choosing $w_d$ and $w_g$ one needs to be aware of the trade-off introduced.
While higher $w_g$ ensures persistence of global statistics it also introduces artifacts as a result of pooling $\hat{\x}_d$ before subtensor embedding and vice versa. 
Higher $w_d$ lays larger emphasis on details while possibly violating global structure.
This trade-off is further influenced by the number of poolings $Q$.

\section{Conclusion} \label{sec:concl}
We present a patch-based approach for image inpainting of high resolution textures using CNN texture synthesis.
Our method is capable of filling large inpainting regions that are visually coherent in global structure as well as details.
We also introduce a distance metric for the comparison of patches based on summary statistics by using masked Gramians.
For future work we plan to develop our method further for inpainting of natural scences. We would also like to apply this concept to 3D surface reconstruction.

\begin{figure*}[tb]
\centering
\subfloat[]{
\includegraphics[width=0.29\textwidth]{images/dots_orig_cutout_small.jpg}
\label{fig:dots}
}
\subfloat[]{
\includegraphics[width=0.29\textwidth]{images/bricks_orig_cutout_small.jpg}
\label{fig:bricks}
}
\subfloat[]{
\includegraphics[width=0.29\textwidth]{images/wood_orig_cutout_small.jpg}
\label{fig:wood}
}
\vspace{-1em}
\newline
\subfloat[]{
\includegraphics[width=0.29\textwidth]{images/dots_pmri_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/bricks_pmri_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/wood_pmri_cut.jpg}
\label{fig:pmri}
}
\vspace{-1em}
\newline
\subfloat[]{
\includegraphics[width=0.29\textwidth]{images/dots_crimi_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/bricks_crimi_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/wood_crimi_cut.jpg}
\label{fig:crimi}
}
\vspace{-1em}
\newline
\subfloat[]{
\hspace{-2em}
\includegraphics[width=0.29\textwidth]{images/dots_ps_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/bricks_ps_cut.jpg}
\hspace{0.06em}
\includegraphics[width=0.29\textwidth]{images/wood_ps_cut.jpg}
\label{fig:ps}
}
\vspace{-1em}
\caption{\protect\subref{fig:dots}-\protect\subref{fig:wood} Original with inpainting region $\Omega$. Close-up on inpainting results of \protect\subref{fig:pmri} PITS, \protect\subref{fig:crimi} EBI, and \protect\subref{fig:ps} PSCS7.}
\label{fig:results}
\end{figure*}


==> relwork.tex <==
\section{Related works} \label{sec:relwork}
Most image inpainting approaches are based on sampling existing information surrounding the inpainting region, wich is called exemplar-based \cite{criminisi2004region, wexler2007space, kwatra2005texture, efros1999texture, kwatra2003graphcut, efros2001image, barnes2009patchmatch} inpainting.
Many exemplar-based methods approach inpainting in a copy-paste fashion.
A very well known method is the work by Criminisi et al. \cite{criminisi2004region} which applies this methodology but restricts the fill order to propagate linear structures (isophotes) first.
This process has been further improved by Barnes et al. \cite{barnes2009patchmatch} who contribute a fast way for randomized correspondence search to find suitable patches.
These approaches are very dependent on patch-size and fail to satisfy global statistics that are not captured within a single patch.
This is a problem since texture is defined as the repetition of simpler elements together with some stochasticity of global repetitions as well as local sub-patterns.
Recently deep learning approaches have been applied successfully to the problems of texture synthesis and image inpainting \cite{li2016combining, gatys2016image, johnson2016perceptual, dosovitskiy2016generating}.
First introduced by Gatys et al. in \cite{gatys2015texture} texture synthesis by CNNs has shown to surpass well known methods like \cite{portilla2000parametric} for many different examples.
Wallis et al. \cite{wallis2017parametric} recently showed that artificial images produced from a parametric texture model closely match texture appearance for humans. Especially, the CNN texture model of \cite{gatys2015texture} and the extension by Liu \cite{liu2016texture} are able to capture important aspects of material perception in humans. For many textures the synthesis results are indiscriminable under foveal inspection.
Other methods like the already mentioned methods by Phatak et al. \cite{pathak2016context} and Yang et al. \cite{yang2016high} train auto-encoder like networks called context-encoders for inpainting. They use a combination of classic pixel-wise reconstruction loss as well as an adversarial loss term and a detail transfer network.



==> suplmatforincl.tex <==
\clearpage
\begin{table*}
\begin{center}
\begin{large}
Supplementary Material
\end{large}
\end{center}
\noindent
Further inpainting results ($2048$x$2048$) of our approach: \subref{fig:mud1} Original with inpainting region $\Omega$ ($512$x$512$), \subref{fig:mud2} result of inpainting global structure (stage one), \subref{fig:mud3} final inpainting result, \subref{fig:mud4} close-up of the inpainted region. 
\end{table*}

%\thanks{This research is funded by the Federal Ministry of Education and Research (BMBF) of Germany (project number 02P14A035).}



\begin{figure*}[htb]
\centering
\hspace{0.2em}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/mud1_small.jpg}
\label{fig:mud1}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/mud2_small.jpg}
\label{fig:mud2}
}
\newline
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/mud3_small.jpg}
\label{fig:mud3}
}
%\hspace{0.1em}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/mud4_small.jpg}
\label{fig:mud4}
}
\vspace{-1em}
\caption{}
\label{fig:results}
\end{figure*}


\begin{figure*}[htb]
\centering
\hspace{0.2em}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/glass1_small.jpg}
\label{fig:mud1}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/glass2_small.jpg}
\label{fig:mud2}
}
\newline
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/glass3_small.jpg}
\label{fig:mud3}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/glass4_small.jpg}
\label{fig:mud4}
}
\vspace{-1em}
\caption{}
\label{fig:results}
\end{figure*}

\begin{figure*}[htb]
\centering
\hspace{0.2em}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/ivy1_small.jpg}
\label{fig:mud1}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/ivy2_small.jpg}
\label{fig:mud2}
}
\newline
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/ivy3_small.jpg}
\label{fig:mud3}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{suplimages/ivy4_small.jpg}
\label{fig:mud4}
}
\vspace{-1em}
\caption{}
\label{fig:results}
\end{figure*}

